In-Context Data Distillation with TabPFN

Foundation models have revolutionized tasks in computer vision and natural language processing. However, in the realm of tabular data, tree-based models like XGBoost continue to dominate. TabPFN, a transformer model tailored for tabular data, mirrors recent foundation models in its exceptional in-context learning capability, being competitive with XGBoost's performance without the need for task-specific training or hyperparameter tuning. Despite its promise, TabPFN's applicability is hindered by its data size constraint, limiting its use in real-world scenarios. To address this, we present in-context data distillation (ICD), a novel methodology that effectively eliminates these constraints by optimizing TabPFN's context. ICD efficiently enables TabPFN to handle significantly larger datasets with a fixed memory budget, improving TabPFN's quadratic memory complexity but at the cost of a linear number of tuning steps. Notably, TabPFN, enhanced with ICD, demonstrates very strong performance against established tree-based models and modern deep learning methods on 48 large tabular datasets from OpenML.

==> figures/tables/auc_table.tex <==
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrr}
\toprule
  & RandomForest & TabPFN Distillation & TabNet & TabPFN Baseline & XGBoost (Default) & XGBoost (Tuned) \\
dataset &  &  &  &  &  &  \\
\midrule
 Amazon-employee-access 34539 & 0.732 & 0.759 & 0.721 & 0.670 & 0.805 & 0.866 \\
 Click-prediction-small 190408 & 0.668 & 0.639 & 0.599 & 0.619 & 0.680 & 0.652 \\
 GesturePhaseSegmentationProcessed 14969 & 0.788 & 0.845 & 0.778 & 0.775 & 0.864 & 0.902 \\
 JapaneseVowels 3510 & 0.980 & 1.000 & 1.000 & 0.997 & 0.999 & 1.000 \\
 MagicTelescope 3954 & 0.897 & 0.924 & 0.938 & 0.923 & 0.937 & 0.939 \\
 MiniBooNE 168335 & 0.958 & 0.979 & 0.939 & 0.951 & 0.979 & 0.984 \\
 PhishingWebsites 14952 & 0.979 & 0.992 & 0.994 & 0.983 & 0.992 & 0.995 \\
 Satellite 167211 & 0.993 & 0.993 & 0.908 & 0.991 & 0.994 & 0.988 \\
 ada-agnostic 3896 & 0.882 & 0.888 & 0.879 & 0.885 & 0.894 & 0.883 \\
 adult-census 3953 & 0.899 & 0.889 & 0.906 & 0.885 & 0.923 & 0.914 \\
 adult 7592 & 0.902 & 0.900 & 0.915 & 0.898 & 0.929 & 0.927 \\
 artificial-characters 14964 & 0.915 & 0.972 & 0.962 & 0.951 & 0.973 & 0.995 \\
 bank-marketing 14965 & 0.900 & 0.906 & 0.933 & 0.889 & 0.927 & 0.927 \\
 cardiotocography 9979 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
 churn 167141 & 0.859 & 0.876 & 0.899 & 0.866 & 0.857 & 0.857 \\
 connect-4 146195 & 0.717 & 0.875 & 0.878 & 0.643 & 0.832 & 0.909 \\
 eeg-eye-state 14951 & 0.856 & 0.990 & 0.685 & 0.969 & 0.953 & 0.987 \\
 electricity 219 & 0.864 & 0.937 & 0.900 & 0.854 & 0.933 & 0.981 \\
 elevators 3711 & 0.841 & 0.936 & 0.935 & 0.932 & 0.917 & 0.928 \\
 eye-movements 3897 & 0.747 & 0.786 & 0.777 & 0.735 & 0.826 & 0.893 \\
 first-order-theorem-proving 9985 & 0.754 & 0.781 & 0.717 & 0.739 & 0.806 & 0.810 \\
 house-16H 3686 & 0.924 & 0.947 & 0.918 & 0.924 & 0.951 & 0.951 \\
 jannis 168330 & 0.771 & 0.819 & 0.849 & 0.771 & 0.840 & 0.848 \\
 jungle-chess 167119 & 0.872 & 0.979 & 0.978 & 0.919 & 0.952 & 0.970 \\
 kc1 3917 & 0.810 & 0.823 & 0.806 & 0.826 & 0.789 & 0.825 \\
 kr-vs-kp 3 & 0.994 & 1.000 & 0.996 & 0.999 & 1.000 & 1.000 \\
 magic 146206 & 0.897 & 0.927 & 0.936 & 0.915 & 0.937 & 0.939 \\
 mfeat-fourier 14 & 0.975 & 0.976 & 0.973 & 0.976 & 0.983 & 0.980 \\
 mfeat-karhunen 16 & 0.992 & 0.998 & 0.998 & 0.993 & 0.997 & 0.997 \\
 mfeat-morphological 18 & 0.942 & 0.951 & 0.954 & 0.951 & 0.945 & 0.939 \\
 mfeat-zernike 22 & 0.963 & 0.978 & 0.978 & 0.980 & 0.969 & 0.964 \\
 mushroom 24 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
 numerai28.6 167120 & 0.525 & 0.526 & 0.511 & 0.515 & 0.522 & 0.508 \\
 nursery 9892 & 0.943 & 1.000 & 0.998 & 0.996 & 1.000 & 1.000 \\
 optdigits 28 & 0.996 & 0.999 & 0.998 & 0.998 & 1.000 & 1.000 \\
 ozone-level-8hr 9978 & 0.933 & 0.945 & 0.914 & 0.945 & 0.910 & 0.920 \\
 page-blocks 30 & 0.962 & 0.967 & 0.951 & 0.971 & 0.984 & 0.968 \\
 pendigits 32 & 0.996 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
 phoneme 9952 & 0.909 & 0.954 & 0.931 & 0.922 & 0.945 & 0.963 \\
 pollen 3735 & 0.489 & 0.462 & 0.499 & 0.462 & 0.507 & 0.480 \\
 satimage 2074 & 0.975 & 0.988 & 0.985 & 0.984 & 0.988 & 0.990 \\
 segment 146822 & 0.987 & 0.993 & 0.991 & 0.994 & 0.994 & 0.994 \\
 shuttle 146212 & 1.000 & 1.000 & 0.977 & 0.999 & 1.000 & 1.000 \\
 spambase 43 & 0.963 & 0.978 & 0.971 & 0.971 & 0.983 & 0.984 \\
 splice 45 & 0.989 & 0.967 & 0.981 & 0.957 & 0.992 & 0.994 \\
 sylvine 168912 & 0.958 & 0.967 & 0.953 & 0.964 & 0.976 & 0.980 \\
 wall-robot-navigation 9960 & 0.996 & 0.988 & 0.996 & 0.973 & 1.000 & 1.000 \\
 wilt 146820 & 0.982 & 0.994 & 0.993 & 0.996 & 0.990 & 0.989 \\
\toprule
median & 0.928 & 0.967 & 0.939 & 0.951 & 0.953 & \textbf{0.969} \\
\bottomrule
\end{tabular}
}

